Robust Deep Reinforcement Learning against Adversarial Perturbations on State Observations

A deep reinforcement learning (DRL) agent observes its states through observations, which may contain natural measurement errors or adversarial noises. Since the observations deviate from the true states, they can mislead the agent into making suboptimal actions. Several works have shown this vulnerability via adversarial attacks, but existing approaches on improving the robustness of DRL under this setting have limited success and lack for theoretical principles. We show that naively applying existing techniques on improving robustness for classification tasks, like adversarial training, is ineffective for many RL tasks. We propose the state-adversarial Markov decision process (SA-MDP) to study the fundamental properties of this problem, and develop a theoretically principled policy regularization which can be applied to a large family of DRL algorithms, including proximal policy optimization (PPO), deep deterministic policy gradient (DDPG) and deep Q networks (DQN), for both discrete and continuous action control problems. We significantly improve the robustness of PPO, DDPG and DQN agents under a suite of strong white box adversarial attacks, including new attacks of our own. Additionally, we find that a robust policy noticeably improves DRL performance even without an adversary in a number of environments. Our code is available at https://github.com/chenhongge/StateAdvDRL.

==> Intro.tex <==
\vspace{-0.5em}
\section{Introduction}
\vspace{-0.5em}
% Deep Q-learning (DQN)~\citep{mnih2015human} achieves human-level performance on many Atari game environments. DQN uses a neural network functional approximator $f(s)$ to estimate the state-action value $Q(s,a)$: given an input frame $(s)$, the neural network predict each action's value. Many variants of DQN has been developed to further improve its performance, including prioritized experience replay, DoubleDQN to improve training stability, DuelingDQN, NoisyNet to allow better exploration
With deep neural networks (DNNs) as powerful function approximators, deep reinforcement learning (DRL) has achieved great success on many complex tasks~\citep{mnih2015human,lillicrap2015continuous,schulman2015trust,silver2016mastering,gu2016continuous} and even on some safety-critical applications (e.g., autonomous driving~\citep{voyage,sallab2017deep,pan2017virtual}).
%Among them, Deep Q Networks (DQN)~\citep{mnih2015human} and Deep Deterministic Policy Gradient algorithms (DDPG)~\citep{lillicrap2015continuous} have become the roots of many enhanced algorithms~\citep{wang2015dueling,hessel2018rainbow,lowe2017multi,fujimoto2018addressing,barth2018distributed}. 
Despite achieving super-human level performance on many tasks, the existence of adversarial examples~\citep{szegedy2013intriguing} in DNNs and many successful attacks to DRL~\citep{huang2017adversarial,behzadan2017vulnerability,lin2017tactics,pattanaik2018robust,xiao2019characterizing} motivates us to study robust DRL algorithms.


% When an RL agent obtains its current state via observations, the observations may contain uncertainty that naturally originates from unavoidable sensor errors or equipment inaccuracy. A policy not robust to such uncertainty can lead to catastrophic failures (Figure~\ref{fig:example_uncertainty}). 
% To ensure safety under the \emph{worst case} uncertainty, in our paper, we consider the adversarial setting where the observation is adversarially perturbed from $s$ to $\nu(s)$, yet the underlying true environment state $s$ where the agent locates is unchanged. 
% This setting is aligned with many adversarial attacks on state observations (e.g., \citep{huang2017adversarial,lin2017tactics}).

% Moreover, DRL agents can be brittle even without any adversarial attacks -- an agent may fail occasionally but catastrophically during regular (non-adversarial) rollouts, and debugging these failure cases can be quite challenging~\citep{uesato2018rigorous}. In Figure~\ref{fig:clean_worst_case}, we show a few DDPG agents achieving high median rewards. However, during 100 episodes (each episode is randomly initialized with a small noise added in OpenAI Gym) we observe occasional low reward runs. In practical applications, such a small noise can be naturally prevalent and thus threaten the use of DRL in safety critical domains.
% % To obtain a better theoretical understanding, we first consider a Markov Decision Process (MDP) under the existence of an optimal adversary for perturbing state observations (named SA-MDP). We derive the basic policy evaluation algorithm and discuss a few unusual properties of SA-MDP: an optimal policy may not exist for SA-MDP, however we can bound the loss of expected reward for a given MDP policy $\pi$. From the analysis of SA-MDP, we provide connections to DRL in both discrete and continuous action spaces. We derive theoretically principled robustness regularizers for DQN and DDPG which are related to an upper bound on performance loss.
% Therefore, it is urgent to improve the robustness of current RL agents under the adversarial (worst) settings now. However, it is a non-trivial problem. A natural approach is to extend the existing adversarial defenses for supervised learning, e.g., adversarial training~\citep{kurakin2016adversarial,madry2017towards,zhang2019theoretically} to DRL.
% % Specifically, we can attack the agent and generate trajectories adversarially during training time, and apply any existing DRL algorithm to hopefully obtain a robust policy. 
% Unfortunately, we show that for most environments, naive adversarial training can make training unstable and deteriorate agent performance (a similar observation is made in~\citep{behzadan2017whatever,fischer2019online}), or does not significantly improve robustness against strong attacks. Since RL and supervised learning are quite different problems, naively applying techniques from supervised learning to RL without a proper theoretical justification can be unsuccessful.

% \setlength{\textfloatsep}{8pt}
% \setlength{\floatsep}{5pt}
% \begin{figure}[t]
% \centering
% \begin{minipage}{.48\textwidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{fig/car_driving.pdf}
%     \caption{A car observes its location through sensors (e.g., GPS) and plans its route to the goal. Without considering the uncertainty in observed location (e.g., error of GPS coordinates), an unsafe policy may crash into the wall because the observed location and true location differ.}
%     \label{fig:example_uncertainty}
% \end{minipage}%
% \hfill
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=0.8\linewidth]{fig/clean_boxplot.pdf}
%   \captionof{figure}{Box plots of rewards over 100 episodes on four Mujoco environments. Even in natural environments {\it without an adversary}, the {\it minimum rewards} DDPG agents receive can be much lower than the median. Our robust SA-DDPG agents obtain much better worst case performance.}
%   \label{fig:clean_worst_case}
% \end{minipage}
% \end{figure}


% In this paper,
% % we focus on the robustness in state observations of RL agents and propose the state-adversarial Markov decision process (SA-MDP) Our SA-DDPG agents trained on a robust policy optimization objective can obtain significantly better worst case reward with much less variance. To summarize, 
% we study the theory and practice of robust RL against perturbations on state observations:

When an RL agent obtains its current state via observations, the observations may contain uncertainty that naturally originates from unavoidable sensor errors or equipment inaccuracy. A policy not robust to such uncertainty can lead to catastrophic failures (e.g., the navigation setting in  Figure~\ref{fig:example_uncertainty}). 
To ensure safety under the \emph{worst case} uncertainty, in our paper we consider the adversarial setting where the state observation is adversarially perturbed from $s$ to $\nu(s)$, yet the underlying true environment state $s$ where the agent locates is unchanged. 
This setting is aligned with many adversarial attacks on state observations (e.g., \citep{huang2017adversarial,lin2017tactics}).
% To obtain a better theoretical understanding, we first consider a Markov Decision Process (MDP) under the existence of an optimal adversary for perturbing state observations (named SA-MDP). We derive the basic policy evaluation algorithm and discuss a few unusual properties of SA-MDP: an optimal policy may not exist for SA-MDP, however we can bound the loss of expected reward for a given MDP policy $\pi$. From the analysis of SA-MDP, we provide connections to DRL in both discrete and continuous action spaces. We derive theoretically principled robustness regularizers for DQN and DDPG which are related to an upper bound on performance loss.
To improve robustness under this setting, a natural approach is to extend existing adversarial defenses for supervised learning, e.g., adversarial training~\citep{kurakin2016adversarial,madry2017towards,zhang2019theoretically} to DRL.
Specifically, we can attack the agent and generate trajectories adversarially during training time, and apply any existing DRL algorithm to hopefully obtain a robust policy. Unfortunately, we show that for most environments, naive adversarial training can make training unstable and deteriorate agent performance (a similar observation is made in~\citep{behzadan2017whatever,fischer2019online}), or does not significantly improve robustness under strong attacks. Since RL and supervised learning are quite different problems, naively applying techniques from supervised learning to RL without a proper theoretical justification can be unsuccessful.

\setlength{\textfloatsep}{13pt}
\setlength{\floatsep}{13pt}
\begin{figure}[t]
\centering
\begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/car_driving.pdf}
    \caption{A car observes its location through sensors (e.g., GPS) and plans its route to the goal. Without considering the uncertainty in observed location (e.g., error of GPS coordinates), an unsafe policy may crash into the wall because the observed location and true location differ.}
    \label{fig:example_uncertainty}
\end{minipage}%
\hfill
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{fig/clean_boxplot.pdf}
  \captionof{figure}{Box plots of rewards over 100 episodes on four Mujoco environments. Even in natural environments {\it without an adversary}, the {\it minimum rewards} DDPG agents receive can be much lower than the median. Our robust SA-DDPG agents obtain much better worst case performance.}
  \label{fig:clean_worst_case}
\end{minipage}
\end{figure}

Additionally, DRL agents can be brittle even without any adversarial attacks -- an agent may fail occasionally but catastrophically during regular (non-adversarial) rollouts, and debugging these failure cases can be quite challenging~\citep{uesato2018rigorous}. In Figure~\ref{fig:clean_worst_case} we show a few DDPG agents achieving high median rewards. However, during 100 episodes (each episode is randomly initialized with a small noise added in OpenAI Gym) we observe occasional low reward runs. In practical applications, such a small noise can be naturally prevalent and thus prohibits the use of DRL in safety critical domains like autonomous driving. The agents trained using our proposed robust policy optimization objective (SA-DDPG) can obtain significantly better worst case reward with much less variance. To summarize, our paper studies the theory and practice of robust RL against perturbations on state observations:
\begin{itemize}[wide,itemsep=0pt]
    \item We formulate the perturbation on state observations as a modified Markov decision process (MDP), which we call state-adversarial MDP (SA-MDP), and study its fundamental properties. We show that under an optimal adversary, a stationary and Markovian optimal policy may not exist for SA-MDP.
    \item Based on our theory of SA-MDP, we propose a theoretically principled robust policy regularizer which is related to the total variation distance or KL-divergence on perturbed policies. It can be practically and efficiently applied to a wide range of RL algorithms, including PPO, DDPG and DQN.
    \item We conduct experiments on 11 environments ranging from Atari games with discrete actions to complex control tasks in continuous action space. Our proposed method significantly improves robustness under strong white-box attacks on state observations, including two \emph{strong} attacks we design, the robust SARSA attack (RS attack) and maximal action difference attack (MAD attack). 
\end{itemize}

%Additionally, we demonstrate that we can achieve better performance than baselines under environment parameter changes (e.g., changes in mass and friction). 
% Moreover, since our method utilizes certifiable neural network training as a keystone, we can obtain certain robustness guarantees for the learned policy.


==> old_dqn_tab.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}\toprule
\multirow{2}{*}{Environment}&\multirow{2}{*}{$\epsilon$}&\multicolumn{3}{c}{DQN}&\multicolumn{3}{|c}{DQN with PGD adversarial training (ratio 0.5)}&\multicolumn{3}{|c}{SA-DQN}&\multicolumn{2}{|c}{\citet{fischer2019online}}\\
&&\shortstack{Natural\\Reward} & \shortstack{PGD Attack\\Reward} &\shortstack{Action\\Cert. Rate}&\shortstack{Natural\\Reward} & \shortstack{PGD Attack\\Reward} &\shortstack{Action\\Cert. Rate}& \shortstack{Natural\\Reward} & \shortstack{PGD Attack\\Reward}&\shortstack{Action\\Cert. Rate}&\shortstack{Natural\\Reward} & \shortstack{PGD Attack\\Reward}\\
\midrule
Pong &1/255 &  20.7 $\pm$ 0.5  & -21.0$\pm$0.0  &  0.0   & 10.1 $\pm$ 6.6  & -21.0 $\pm$ 0.0 &  0.0   &21.0 $\pm$ 0.0 & \bf 20.1 $\pm$ 0.0  &   1.000 &19.73&18.13\\\hline%&  0.002
Freeway &1/255&  32.9 $\pm$ 0.7  & 0.0 $\pm$ 0.0 & 0.0   & 25.4    $\pm$ 0.8  & 0.0$\pm$ 0.0 &0.0     &30.78 $\pm$ 0.5  &  30.36 $\pm$ 0.7 &   0.995  &32.93& \textbf{32.53}\\\hline%&   0.0001
BankHeist &1/255 &  1308.4 $\pm$ 24.1  &  56.4 $\pm$ 21.2 &  0.0  &  1126.0  $\pm$  70.9  & 9.4  $\pm$ 13.6 &  0.0   &1041.4 $\pm$ 12.3  &  \bf 1043.6 $\pm$ 9.5 &  0.997 &238.66&190.67\\\hline%&   0.01
RoadRunner &1/255 &  36946.0 $\pm$ 6089.0  & 0.0 $\pm$ 0.0 &  0.0  &  22944.0 $\pm$ 6532.5  &14.0 $\pm$ 34.7 &   0.0  &15172.0 $\pm$ 791.7  & \bf 15280.0 $\pm$ 827.7  &  0.969   &12106.67&5753.33\\\hline%&   0.003
% CartPole &0.2 std  &  &   &   &    &   &   &     \\
Acrobot &0.2 std & -67.5 $\pm$ 8.8 & -349.7 $\pm$ 178.0  & 0.735    &  -82.8  $\pm$  9.9 & -155.1 $\pm$ 79.6 &  0.718   &  -79.4 $\pm$ 17.4& \bf -86.7 $\pm$ 19.9  &  0.856   &-&-\\%&  0.005
\bottomrule
\end{tabular}
}
\caption{Average test reward values and action certification rates over 50 episodes with and without test time PGD attacks on regular DQN, PGD adversarially trained DQN with adversarial ratio 0.5, and SA-DQN models. Natural reward is the reward in clean environment without adversarial attacks. Attack reward is the reward under PGD attacks on state observations. Action Cert. Rate is the proportion of the actions that are guaranteed and cannot be changed by any attacks within given $\epsilon$. We also include the state-of-the-art results from~\citet{fischer2019online}.}
\label{tab:dqn_res_t}
\end{table*}


==> tables/ddpg_fig_table.tex <==
\begin{figure*}[t!]
    \centering
\begin{subfigure}[t]{.32\linewidth}
    	\centerline{    \includegraphics[width=\columnwidth]{fig/tmp_halfcheetah_friction.png}
}
        \caption{HalfCheetah}
    \end{subfigure}
    \begin{subfigure}[t]{.32\linewidth}
    	\centerline{    \includegraphics[width=\columnwidth]{fig/tmp_hopper_friction.png}
}
        \caption{Hopper}
    \end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
    	\centerline{    \includegraphics[width=\columnwidth]{fig/tmp_ant_friction.png}
}
        \caption{Ant}
    \end{subfigure}
    
    
    \begin{subfigure}[t]{.32\linewidth}
    	\centerline{    \includegraphics[width=\columnwidth]{fig/tmp_invertedpendulum_length.png}
}
        \caption{InvertedPendulum}
    \end{subfigure}
    \begin{subfigure}[t]{.32\linewidth}
    	\centerline{    \includegraphics[width=\columnwidth]{fig/tmp_hopper_mass.png}
}
        \caption{Hopper}
    \end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
    	\centerline{    \includegraphics[width=\columnwidth]{fig/tmp_ant_mass.png}
}
        \caption{Ant}
    \end{subfigure}
    
    
    % \includegraphics[width=0.32\linewidth]{fig/tmp_hopper_friction.png}
    % \includegraphics[width=0.32\linewidth]{fig/tmp_ant_friction.png}
    % \includegraphics[width=0.32\linewidth]{fig/tmp_invertedpendulum_length.png}
    % \includegraphics[width=0.32\linewidth]{fig/tmp_hopper_mass.png}
    % \includegraphics[width=0.32\linewidth]{fig/tmp_ant_mass.png}
    \caption{Comparison
    between DDPG and SA-DDPG
    on the robustness  to
changing environment dynamics. The dotted line on each figure represents the original environment parameter (friction, length or mass) used during training.}
    \label{fig:overall_randomization}
\end{figure*}


==> tables/ddpg_sigma_noise.tex <==
% \begin{table*}[tbh]\centering
% \caption{Comparison between  Smoothed and Non-smoothed policies on SA-DDPG (Convex) models in Table~\ref{tab:ddpg_res}.  We report mean reward $\pm$ standard deviation over 50 attack episodes.}
% \resizebox{\linewidth}{!}{
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{tabular}{l|c|c|c| c| c}
% \hline
% \multirow{2}{*}{Env.} & \multirow{2}{*}{\shortstack{$\ell_\infty$ norm perturb-\\ation budget $\epsilon$}}                                   & \multirow{2}{*}{\shortstack{Smoothed \\   \textbf{Natural} Reward}}&\multirow{2}{*}{\shortstack{Non-smoothed \\\textbf{Natural} Reward}} & \multirow{2}{*}{\shortstack{Smoothed\\  Best \textbf{Attack} Reward}}&\multirow{2}{*}{\shortstack{Non-smoothed \\Best \textbf{Attack} Reward}}\\
%                       &                                                              &                         &                                   & \\ \hline
% %   &  &  390.18 $\pm$ 472.07 & \bf 367.74 $\pm$ 346.33 \\
%  Ant  & 0.2 & 2129.70 $\pm$ 60.54 &  2111.22 $\pm$ 158.88 & 1963.91 $\pm$ 56.19 & 1958.79 $\pm$ 105.24 \\
% % \hline
% %  HalfCheetah  &  & 5625.93 $\pm$ 1509.95 &  7546.38 $\pm$ 91.69 & 952.25 $\pm$ 946.80 & 1118.58 $\pm$ 867.50 \\
% \hline
%  Hopper  & 0.075 & 3348.96 $\pm$ 516.18 &  3496.25 $\pm$ 30.84 & 1555.24 $\pm$ 953.33 & 1603.90 $\pm$ 589.46 \\
% \hline
%  InvertedPendulum  & 0.5 & 1000.00 $\pm$ 0.00 &  1000.00 $\pm$ 0.00 & 800.98 $\pm$ 329.25 & 877.86 $\pm$ 279.33 \\
% \hline
%  Reacher  & 1.5 & -5.43 $\pm$ 2.26 &  -5.22 $\pm$ 2.12 & -12.51 $\pm$ 4.74 & -13.86 $\pm$ 3.82 \\
% \hline
%  Walker2d  &  0.15 & 3379.16 $\pm$ 1433.54 &  4234.60 $\pm$ 853.86 & 2079.65 $\pm$ 1069.95 & 1944.77 $\pm$ 1143.25 \\
% \hline


% \end{tabular}
% }
% \label{tab:noise_ddpg}
% \end{table*}



\begin{table*}[tbh]\centering
\caption{Comparison between  Smoothed and Non-smoothed policies on SA-DDPG (Convex) models in Table~\ref{tab:ddpg_res}.  We report mean reward $\pm$ standard deviation over 50 attack episodes.}
\resizebox{\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|c|c|c| c| c}
\hline
\multirow{2}{*}{Env.} & \multirow{2}{*}{\shortstack{$\ell_\infty$ norm perturb-\\ation budget $\epsilon$}}                                   & \multirow{2}{*}{\shortstack{Smoothed \\   \textbf{Natural} Reward}}&\multirow{2}{*}{\shortstack{Non-smoothed \\\textbf{Natural} Reward}} & \multirow{2}{*}{\shortstack{Smoothed\\  Best \textbf{Attack} Reward}}&\multirow{2}{*}{\shortstack{Non-smoothed \\Best \textbf{Attack} Reward}}\\
                      &                                                              &                         &                                   & \\ \hline
%   &  &  390.18 $\pm$ 472.07 & \bf 367.74 $\pm$ 346.33 \\
 Ant  & 0.2 & $2263 \pm 491$  & $2254 \pm 430$  & $1793 \pm 1793$  & $1826 \pm 1826$  \\
% \hline
%  HalfCheetah  &  & 5625.93 $\pm$ 1509.95 &  7546.38 $\pm$ 91.69 & 952.25 $\pm$ 946.80 & 1118.58 $\pm$ 867.50 \\
\hline
 Hopper  & 0.075 & $2949 \pm 666$  & $3128 \pm 453$  & $1252 \pm 1252$  & $1449 \pm 1449$  \\
\hline
 InvertedPendulum  & 0.5 & $1000 \pm 0$  & $1000 \pm 0$  & $1000 \pm 1000$  & $1000 \pm 1000$  \\
\hline
 Reacher  & 1.5 &$-5 \pm 2$  & $-5 \pm 2$  & $-12 \pm -12$  & $-12 \pm -12$   \\
\hline
 Walker2d  &  0.15 & $3993 \pm 1848$  & $4540 \pm 1562$  & $2008 \pm 2008$  & $2245 \pm 2245$   \\
\hline


\end{tabular}
}
\label{tab:noise_ddpg}
\end{table*}





==> tables/fig_env_change.tex <==
\begin{small}
\begin{table}
\centering
\resizebox{1.0\linewidth}{!}{%

\begin{tabular}{l|c||c|c|c|c}\toprule
\multirow{2}{*}{Environment}&\multirow{2}{*}{$\epsilon$} & \multicolumn{2}{c|}{DDPG}  & \multicolumn{2}{c}{SA-DDPG} \\
& & $\ell_2$ & Range & $\ell_2$ & Range\\ \midrule
\multirow{1}{*}{Ant} & \multirow{1}{*}{0.2} & 4.19 & 1.45 & 0.49&0.16 \\

\hline

\multirow{1}{*}{HalfCheetah} & \multirow{1}{*}{0.5} & 4.73 & 1.92 & 3.22 & 1.06\\

\hline


\multirow{1}{*}{Hopper} & \multirow{1}{*}{0.075}&  2.96 & 1.68& 0.58 & 0.30\\

\hline

\multirow{1}{*}{\shortstack{InvertedPendulum}} & \multirow{1}{*}{0.75} & 1.05 & 1.05& 0.23 & 0.23 \\

\hline


\multirow{1}{*}{Reacher} & \multirow{1}{*}{1.5} & 1.50 & 1.06  & 0.31 & 0.21\\

\hline
\multirow{1}{*}{Walker2d} & \multirow{1}{*}{0.15} & 4.57 & 1.85  &  0.57 & 0.19\\
\bottomrule
\end{tabular}
}
\caption{Certificates of action change given bounded state perturbations. Numbers are averaged over all steps in 10 rollouts. Smaller numbers indicate better certificates.}
\label{tab:ddpg_certificate}
\end{table}
% }
\end{small}
